Model-Based Deep Learning

Signal processing, communications, and control have traditionally relied on classical statistical modeling techniques. Such model-based methods utilize mathematical formulations that represent the underlying physics, prior information and additional domain knowledge. Simple classical models are useful but sensitive to inaccuracies and may lead to poor performance when real systems display complex or dynamic behavior. On the other hand, purely data-driven approaches that are model-agnostic are becoming increasingly popular as datasets become abundant and the power of modern deep learning pipelines increases. Deep neural networks (DNNs) use generic architectures which learn to operate from data, and demonstrate excellent performance, especially for supervised problems. However, DNNs typically require massive amounts of data and immense computational resources, limiting their applicability for some signal processing scenarios. We are interested in hybrid techniques that combine principled mathematical models with data-driven systems to benefit from the advantages of both approaches. Such model-based deep learning methods exploit both partial domain knowledge, via mathematical structures designed for specific problems, as well as learning from limited data. In this article we survey the leading approaches for studying and designing model-based deep learning systems. We divide hybrid model-based/data-driven systems into categories based on their inference mechanism. We provide a comprehensive review of the leading approaches for combining model-based algorithms with deep learning in a systematic manner, along with concrete guidelines and detailed signal processing oriented examples from recent literature. Our aim is to facilitate the design and study of future systems on the intersection of signal processing and machine learning that incorporate the advantages of both domains.

==> backup-text.tex <==
%removed this paragraph and the figure , we have already said that deep learning needs a lot of data and compute and this is also well understood- no need to have a figure also showing that. 

	% paragraph - deep learning is not magic
	Deep learning methods are currently transforming computer vision, speech processing, and natural language processing \cite{brock2018large,redmon2016you,oord2016wavenet,vaswani2017attention,brown2020language}.
	which are areas where accurate tractable handcrafted models are   difficult to obtain. However, despite its enormous success, deep learning is subject to several challenges which limit its applicability in some important scenarios, and specifically setups traditionally studied within the frameworks of signal processing and communications. 
	In particular, end-to-end \acp{dnn} models
	are not hard-coded but learned from data. As such, they require an {\em algorithm} that dictates what to learn and how to do so; a sufficiently large {\em data set} which can be provided for learning purposes; and adequate {\em computational resources} to process the data. An illustration of these key ingredients is depicted in Fig. \ref{fig:ML_triangle}. The fundamental algorithmic foundations of deep learning, such as the use of generic model-agnostic multi-layer neural networks and training by backpropagation, date back  several decades ago (e.g. \cite{widrow199030}). The dramatic success of deep learning over the last few years is thus attributed mostly to the availability of systems with increased computational power, that can maintain and adapt highly-parametrized \acp{dnn}, and the proliferation of data, which is essential for training these networks. In fact, the demands for computational and data resources are growing dramatically as deep learning research progresses. For instance, the current state-of-the-art deep language model GPT-3 consists of 175 billion weights, which is over a hundred times more trainable parameters compared to its predecessor released in 2019 \cite{brown2020language}.
	

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
